Understanding Types of Users on Twitter

People use microblogging platforms like Twitter to involve with other users for a wide range of interests and practices. Twitter profiles run by different types of users such as humans, bots, spammers, businesses and professionals. This research work identifies six broad classes of Twitter users, and employs a supervised machine learning approach which uses a comprehensive set of features to classify users into the identified classes. For this purpose, we exploit users' profile and tweeting behavior information. We evaluate our approach by performing 10-fold cross validation using manually annotated 716 different Twitter profiles. High classification accuracy (measured using AUC, and precision, recall) reveals the significance of the proposed approach.

==> dataCollection.tex <==
% !TEX root = paper.tex


==> featureSet.tex <==
\subsection{Feature Set}

%Twitter users interact using tweets, retweets, statuses and reply to statuses. They use links, hashtags and mentions that adds an additional meaning to tweets like links are used for referencing, hashtags and mentions are for communication/chat. 
%We consider a user's tweeting behavior (tweet, retweet, endorsement, etc.) and external information (links, hashtags, etc.) mentioned in tweets and profile description as a source to classify user under the above defined user categories.
%Consider five features, a mix of profile-based and tweeting behavior-based features -- 1) users without a website in their profile description, 2) users with verified twitter accounts, 3) retweets in each class, 4) endorsement, 5) response to status. 

%For the collected 716 user profiles, we calculate average value of each feature based on the two main classes -- real users and digital actors. Figure 2 shows how these feature help in separating the two main classes. Real users and digital actors have very different behavior for the profile-based feature "verified Twitter account" and a feature based on tweeting behavior "response to status". The real users tend to have more verified accounts and are active in responding to statuses compared to digital actors. We also plot the graph of classes existed inside of each major class. Figure 3 and Figure 4 show the graph of four sub-classes of real users and three sub-classes of digital users respectively. 


%\begin{center}
%\includegraphics[width=\columnwidth]{figs/twoClassGraph.png}
%\label{figure2}
%\hypertarget{figure2}{\tiny Figure.2 Two class distribution using five features} 
%\end{center}
%
%\begin{center}
%\includegraphics[width=\columnwidth]{figs/humanGraph.png}
%\label{figure3}
%\hypertarget{figure3}{\tiny Figure.3 Four classes of real users wrt. some features} 
%\end{center}
%
%\begin{center}
%\includegraphics[width=\columnwidth]{figs/autoGraph.png}
%\label{figure4}
%\hypertarget{figure4}{\tiny Figure.4 Three classes of digital actors wrt. some profile-based and tweeting behavior-based features} 
%\end{center}
%
%It can be seen from figure \ref{figure3} Professional users generally provide URL in their profile description compared to other classes. Combined with personal users, they have verified accounts. All classes show similar behavior in retweeting. Niche and Professional users tend to have higher endorsement ratio compared to other two classes. Personal users have lower average number of response to status compared to other classes. A similar observations can be made from figure \ref{figure4}.

%Bots are not interactive in community; often shows periodic tweeting linked with the content on web source. They are poor in information consumption and social behavior. Though they are broadcasting the news, some of them have special interests or topic based news linked with web sources like web portal or blogs. The bloggers retweet and interactive with other users as compared to news broadcasters. They tend to post tweet redirecting to the content at their blog.

%%Viral users chat and share information. They have a personal character and thought reflection.

%The graph shows that the classes defined in an earlier section of the paper are inline with the profile-based and tweeting behavior-based features.
%
%There are several features available through Twitter API that are related to a user. We restrict ourself to profile-based and tweeting behavior-based features. 

We choose 18 features as summarized in Table \ref{tab:features}.
A horizontal line in the table separates tweet-related features with profile-based features. In the following, we only explain the derived features that are not easily comprehendable.

%\begin{table}[htb]
%\centering
%\small
\begin{center}
\small
\begin{tabular}{l | p{4.0 cm}}
\toprule
Feature & Definition \\
\midrule
Favorites count & No. of favorite action \\
Verified & Verified twitter account \\
Promotion score & Count of URL mentioning user profile name or referenced website in user profile description\\
Life time & Life time of a user till the last tweet \\
\midrule
Plain status & No. of plain statuses \\
Tweet spread/influence & Total retweet status count/total time for 100 tweets (in hour) \\
Response to status & Count of statuses as a reply to other statuses \\
Response to users & Count of response to users\\
Std URLs & Standard deviation of tweets with mentioned URL \\
Std hashtags & Standard deviation of tweets with hashtags\\
Retweeted status count & Response to the other statuses \\
Time Difference & Time difference from last and first tweet in the sample \\
User Actions & Sum of number of tweets, number of following and number of lists per time difference\\
Action inclination & Harmonic mean of personal status and retweeted status \\
Mention count & Number of mentions in sample per time difference\\
Fame actions & Sum of follower count, user listed count and favorite count\\
Total urls  & Sum of all URLS in last 100 tweets\\
Total hashtags & Sum of all hashtags in last 100 tweets\\
\bottomrule
\end{tabular}
\label{tab:features}
\hypertarget{tab:features}{Features used to annotate user profiles}
\end{center}
%\caption{Full feature list used to classify user profiles}
%\label{tab:features}
%\end{table}

In action inclination, we use harmonic mean of personal status and retweeted status to measure the correlation between them. 
%
%was used as it will enhance the effect of two features if they are statistically correlated, where as if they are not correlated, the feature will give a trade off mean, making it a poor feature. Ofcourse, in feature optimization step, some of the feature will be reduced as describe in next section.
%
Promotion score represents the edit distance score between the "expanded$\_$url" and the user profile name. Comparing promotion score with different classes can give interesting insight about self branding or self promotion.

For further improvement, we process data with information gain based feature selection algorithm. We draw out feature aggregates and label user profile by simultaneously observing aggregates and user twitter profile. %We also navigate to her web link in case it is mentioned in the profile. 
The features personal, responsive (reply to others status), tweeting frequency are key terms that are observed in a profile. %Producers share a lot more frequently as compare to consumer, and have low in personal reflection as compare to consumer. There are profiles, which are highly frequent in tweeting activity so much so they can be easily identified as automatic producer. All such users have most domain character is robotic sharing activity.
%
%Profiles sharing personal thoughts are active consumers and when consumers also show responsiveness and interacation, they are labeled as interactive consumer.
%
%Automatic producers were analyzed separately with respect to professional news/magazines distribution services showing almost no interaction and personal character but they posses a professional web resource and reference. Profiles, which are showing association with an online blog/product or service, are feeders. Most of the links they share are directed toward their products or services. Viral users are there to chat and share information. They also have a personal character and thought reflection.
%
%%In terms of two perspectives, we can observe a very complex interaction among all these classes as the time varies. Any of viral activity if slows down, the user consumer behavior will change. Since, the scope of paper does not deal with the dynamics of two perspectives with time, we will focus on it in future work.

Table \ref{tab:classdistribution} shows the total class distribution in the annotated data. We get 37, 550, 19, 228 and 300 user profiles as personal, professional, business, niche, spam, feeds and viral consumer respectively.

%\begin{table}%[htb]
%\centering
%\small
\begin{center}
\begin{tabular}{l | r}
\toprule
Class & Users  \\
\midrule
Personal & 19 \\
Professional & 24 \\
Business & 157 \\
Niche & 375 \\
Spam & 49 \\
Blog/Feed & 51 \\
Viral & 41 \\
\midrule
{\bf Total} & {\bf 716} \\
\bottomrule
\end{tabular}
\label{tab:distribution}
\hypertarget{tab:classdistribution}{Seven Class Distribution}
\end{center}

%The links, mentions in tweets and retweets have social contextual annotation. Links are used for referencing, mentions are used for comunication/chat and retweets represent endorsements. 
%A link in a profile could be of user's profile own mentioned site could be significant where as referencing can also be to other social media apps.


\spara{Results and Discussion}
\note[Imran]{Discuss results a little bit. The aim of this should be to set a ground for our next section (Feature extraction) }

\note[Hassan]{some part of it can go to the description of graphs}

Figures show averages for five (A,B,C,D and E) interesting behavior by each class. News, viral, and feed are similar as they show high tweeting behavior but they have
different implicit behaviors. Similarly, endorsement behavior clearly segregate business user from others. Personal and Viral show great
similarity in personal feature but are different than all. where A = user ratio who do not provide website, B=user ratio who are not verified ,
C=retweet count ratio in each class , D= endorsement ratio and E=response to status ratio.

Here retweet count ratio is the sum of the all the tweet count greater than 10 for each tweet of user. The count actually shows how much
famous is the tweet. More retweet count implies popularity of tweet is also more.
Endorsement ratio is number of times when a user retweet a tweet.

%%\begin{center}
%\includegraphics[width=\columnwidth]{figs/businessvspro-niche.pdf}
%\label{figure2}
%\hypertarget{figure2}{\tiny Figure.2 business versus professional and niche } 
%\end{center}

%\begin{center}
%\includegraphics[width=\linewidth]{figs/newsvsviral.pdf}
%\label{figure2}
%\hypertarget{figure2}{\tiny Figure.2 News versus Viral } 
%\end{center}

